\llinstruct: An Instruction-tuned model for English Language Proficiency Assessments

We present \llinstruct: An 8B instruction-tuned model that is designed to generate content for English Language Proficiency Assessments (ELPA) and related applications. Our work involves creating a new dataset of 70K instructions and explanations in the ELPA domain and using these to fine-tune Llama-3 8B models (SFT) of different sizes (e.g., SFT-17K, SFT-50K and SFT-70K). Human evaluations are conducted over unseen instructions to compare these SFT models against SOTA models (e.g., Dolly-2, Mistral, Llama-3 base version, and GPT-3.5). The findings show although all three SFT models perform comparably, the model trained on largest instruction dataset -- SFT-70K - leads to the most valid outputs ready for assessments. However, although the SFT models perform better than larger model, e.g., GPT 3.5 on the aspect of explanations of outputs, many outputs still need human interventions to make them actual ready for real world assessments.

==> eval_expert_examples.tex <==

\iffalse 
\begin{table*}[!t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{subtable}{1\linewidth}
\begin{tabular}{p{0.5\linewidth}p{0.5\linewidth}}\toprule
Original Item  & Seed Instruction  \\\midrule
& \hangindent=0.5em Instruction: Select the correct response to the following question. \\
& \hangindent=0.5em Input: who is your favorite tennis player? \\
& \hangindent=0.5em Output: I don't like any sports. \\
(1) Choose the best response.& \hangindent=0.5em Explanation: Reply indirectly addresses the question by stating a general disinterest in sports rather than specifically identifying a favorite tennis player. \\
\cline{2-2}
Statement: who is your favorite tennis player? & \hangindent=0.5em Instruction: Write three wrong answers to the question. \\
 &  \hangindent=0.5em Input: who is your favorite tennis player? \\
Answers: [`play the song again', `my favorite color is green', `that sounds like fun',\textbf{`I don't like any sports'}]  & \hangindent=0.5em  Output: [`play the song again', `my favorite color is green', `that sounds like fun']\\
&  Explanation: The given answers are either unrelated (e.g.  ``play the song again''), changing the subject (e.g. talking about a favorite color), or expressing a general sentiment (e.g. commenting on an activity).\\
\midrule


& \hangindent=0.5em Instruction: Write a [passage type = recorded message] around [length = 100 words] from [org = XYZ Auto Shop] to [person = Mr. John] to notify that his car repair was finished early and make arrangements for him to pick up the car. \\
& \hangindent=0.5em Input: no-Input \\
& \hangindent=0.5em Output: Hello Mr. John, this is Thomas from XYZ Auto Shop calling with some information about your car repair \dots  we got the parts early, and I was able to finish the repair. \dots you’re welcome to come get your car anytime tomorrow\dots \\
(2) Refer to the following recorded message.& \hangindent=0.5em Explanation: The passage successfully addressed the context asked by providing Mr. John with information that his car repair was done early \dots \\
\cline{2-2}
Recorded message: Hello Mr. John, this is Thomas from XYZ Auto Shop calling with some information about your car repair \dots  we got the parts early, and I was able to finish the repair. \dots you’re welcome to come get your car anytime tomorrow\dots & \hangindent=0.5em Instruction: Based on the following passage write the correct answer to the question ``What does the speaker say about the repair?'' \\
 Question: What does the speaker say about the repair? &  \hangindent=0.5em Input: Hello Mr. John, this is Thomas from XYZ Auto Shop calling with some information about your car repair \dots  we got the part early, and I was able to finish the repair. \dots you’re welcome to come get your car anytime tomorrow\dots \\
Answers: [`it is not required', `covered by warranty', `\textbf{has been finished early}',{`it will be expensive'}]  & \hangindent=0.5em  Output: it has been finished early.\\
& \hangindent=0.5em  Explanation: The reply directly answers the question by stating that the repair mentioned in the context was completed ahead of the initially expected time.\\
\midrule

 \end{tabular}
 \end{subtable}

\caption{\label{table:seed} A few examples (shortened for brevity) of seed instructions. \textbf{bold} selections depict the correct choices. Original items are lightly edited for anonymity.}
\end{table*}

\fi 

\begin{table*}[th]
\begin{center}
\small
\setlength{\tabcolsep}{4pt}
%\begin{tabularx}{\textwidth}{@{}C{0.5} l L %C{0.7} 
%llll@{}}
\begin{tabular}{@{} p{2.9cm} p{2.9cm} p{2.9cm} p{3cm} ccccc@{}}
% \begin{tabular}{p{3cm}p{1cm}p{3cm}p{1cm}p{1cm}p{1cm}p{1cm}}
% \hline
Instruction  & Input & Output & Explanation &  Val. & ITyp. & InpF. & OutC. & QuaE.   \\ \toprule
%{Reframe the sentence in the subjunctive mood.} & {The world is flat.} & {If the world were flat.} & The sentence is expressing a hypothetical situation. & V & NF & M & R & Y         \\ %\cline{2-7} 
Identify the tone of the following text: formal or informal? &	How's it going, buddy?	& informal &	Use of casual language. & VR & NF & M & R & Y \\ 
Create a question based on the email that asks about the scheduled date for the product launch.	& Email: `\``Dear John, \dots the product launch happening next week. \dots we appreciate all the hard work and dedication \dots Best, Jane\''' &	When is the product launch scheduled?	& The answer correctly specifies a question about the product launch date \dots. & VR & NF & M & R & Y \\
Identify the type of pronoun \dots &	My teachers praise me. & Possessive pronoun and Personal pronoun &  The reply correctly identifies `my' as a possessive pronoun and `me' as a personal pronoun & V	& NF	& DNM	& W	& Y \\
Fill in the [MASK] for the following sentence:  The book is [MASK] the table.	& [on, in, around, beside]	& on	& The response 'on' correctly fits into the blank \dots the other options are not logically correct \dots &		I &	NF &	M &	R	& WN \\
\end{tabular}
\caption{\label{table:eval}Evaluation Examples
}
\end{center}
\end{table*}

